Exploiting Belief Bases for Building Rich Epistemic Structures

We introduce a semantics for epistemic logic exploiting a belief base abstraction. Differently from existing Kripke-style semantics for epistemic logic in which the notions of possible world and epistemic alternative are primitive, in the proposed semantics they are non-primitive but are defined from the concept of belief base. We show that this semantics allows us to define the universal epistemic model in a simpler and more compact way than existing inductive constructions of it. We provide (i) a number of semantic equivalence results for both the basic epistemic language with "individual belief" operators and its extension by the notion of "only believing", and (ii) a lower bound complexity result for epistemic logic model checking relative to the universal epistemic model.

==> eptcsdata.tex <==
\providecommand{\firstpage}{332}
\providecommand{\publicationstatus}{L.S. Moss (Ed.): TARK 2019 \\
EPTCS 297, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.297.21}{10.4204/EPTCS.297.21}}
\pdfoutput=1

